Comparing the Carath\'eodory Pseudo-Distance and the K\"ahler-Einstein Distance on Complete Reinhardt Domains

We show that on a certain class of bounded, complete Reinhardt domains in $\mathbb{C}^n$ that enjoy a lot of symmetries, the Carath\'eodory pseudo-distance and the geodesic distance of the complete K\"ahler-Einstein metric with Ricci curvature $-1$ are different.

==> reference.tex <==
@article {CBY99,
	AUTHOR = {Chen, Bo-Yong},
	TITLE = {Completeness of the {B}ergman metric on non-smooth
	pseudoconvex domains},
	JOURNAL = {Ann. Polon. Math.},
	FJOURNAL = {Annales Polonici Mathematici},
	VOLUME = {71},
	YEAR = {1999},
	NUMBER = {3},
	PAGES = {241--251},
	ISSN = {0066-2216},
	MRCLASS = {32F45 (32F17 32U10)},
	MRNUMBER = {1704301},
	MRREVIEWER = {Zbigniew B\l ocki},
	DOI = {10.4064/ap-71-3-241-251},
	URL = {https://doi.org/10.4064/ap-71-3-241-251},
}

@incollection {MNYST83,
	AUTHOR = {Mok, Ngaiming and Yau, Shing-Tung},
	TITLE = {Completeness of the {K}\"{a}hler-{E}instein metric on bounded
	domains and the characterization of domains of holomorphy by
	curvature conditions},
	BOOKTITLE = {The mathematical heritage of {H}enri {P}oincar\'{e}, {P}art 1
	({B}loomington, {I}nd., 1980)},
	SERIES = {Proc. Sympos. Pure Math.},
	VOLUME = {39},
	PAGES = {41--59},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {1983},
	MRCLASS = {53C55 (32F15 53C25)},
	MRNUMBER = {720056},
	MRREVIEWER = {Hung-Hsi Wu},
}

@book {K70,
	AUTHOR = {Kobayashi, Shoshichi},
	TITLE = {Hyperbolic manifolds and holomorphic mappings},
	SERIES = {Pure and Applied Mathematics},
	VOLUME = {2},
	PUBLISHER = {Marcel Dekker, Inc., New York},
	YEAR = {1970},
	PAGES = {ix+148},
	MRCLASS = {32.60},
	MRNUMBER = {0277770},
	MRREVIEWER = {W. Kaup},
}

@incollection {DKFJEHG84,
	AUTHOR = {Diederich, K. and Forn\ae ss, J. E. and Herbort, G.},
	TITLE = {Boundary behavior of the {B}ergman metric},
	BOOKTITLE = {Complex analysis of several variables ({M}adison, {W}is.,
	1982)},
	SERIES = {Proc. Sympos. Pure Math.},
	VOLUME = {41},
	PAGES = {59--67},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {1984},
	MRCLASS = {32H15 (32E35 32F15)},
	MRNUMBER = {740872},
	MRREVIEWER = {I. P. Ramadanov},
	DOI = {10.1090/pspum/041/740872},
	URL = {https://doi.org/10.1090/pspum/041/740872},
}

@article {KLE78,
	AUTHOR = {Klembeck, Paul F.},
	TITLE = {K\"{a}hler metrics of negative curvature, the {B}ergmann metric
	near the boundary, and the {K}obayashi metric on smooth
	bounded strictly pseudoconvex sets},
	JOURNAL = {Indiana Univ. Math. J.},
	FJOURNAL = {Indiana University Mathematics Journal},
	VOLUME = {27},
	YEAR = {1978},
	NUMBER = {2},
	PAGES = {275--282},
	ISSN = {0022-2518},
	MRCLASS = {32F15 (32H15 53C55)},
	MRNUMBER = {463506},
	MRREVIEWER = {Hung-Hsi Wu},
	DOI = {10.1512/iumj.1978.27.27020},
	URL = {https://doi.org/10.1512/iumj.1978.27.27020},
}

@article {AHPJD12
	AUTHOR = {Ahn, Heungju and Park, Jong-Do},
	TITLE = {The explicit forms and zeros of the {B}ergman kernel function for {H}artogs type domains},
	JOURNAL = {J. Funct. Anal.},
	FJOURNAL = {Journal of Functional Analysis},
	VOLUME = {262},
	YEAR = {2012},
	NUMBER = {8},
	PAGES = {3518--3547},
	ISSN = {0022-1236},
	MRCLASS = {32A25 (32A07 32M15)},
	MRNUMBER = {2889166},
	MRREVIEWER = {Atsushi Yamamori},
	DOI = {10.1016/j.jfa.2012.01.021},
	URL = {https://doi.org/10.1016/j.jfa.2012.01.021},
}

@article {WU73,
	AUTHOR = {Wu, H.},
	TITLE = {A remark on holomorphic sectional curvature},
	JOURNAL = {Indiana Univ. Math. J.},
	FJOURNAL = {Indiana University Mathematics Journal},
	VOLUME = {22},
	YEAR = {1972/73},
	PAGES = {1103--1108},
	ISSN = {0022-2518},
	MRCLASS = {53C55},
	MRNUMBER = {315642},
	MRREVIEWER = {Y. Mut\^{o}},
	DOI = {10.1512/iumj.1973.22.22092},
	URL = {https://doi.org/10.1512/iumj.1973.22.22092},
}

@article {BT16-2,
	AUTHOR = {Beberok, Tomasz},
	TITLE = {Explicit formulas of the {B}ergman kernel for some {R}einhardt	domains},
	JOURNAL = {J. Geom. Anal.},
	FJOURNAL = {Journal of Geometric Analysis},
	VOLUME = {26},
	YEAR = {2016},
	NUMBER = {4},
	PAGES = {2883--2892},
	ISSN = {1050-6926},
	MRCLASS = {32A25 (33D70)},
	MRNUMBER = {3544944},
	MRREVIEWER = {Luke David Edholm},
	DOI = {10.1007/s12220-015-9652-0},
	URL = {https://doi.org/10.1007/s12220-015-9652-0},
}

@article {BT16,
	AUTHOR = {Beberok, Tomasz},
	TITLE = {Lu {Q}i-{K}eng's problem for intersection of two complex
	ellipsoids},
	JOURNAL = {Complex Anal. Oper. Theory},
	FJOURNAL = {Complex Analysis and Operator Theory},
	VOLUME = {10},
	YEAR = {2016},
	NUMBER = {5},
	PAGES = {943--951},
	ISSN = {1661-8254},
	MRCLASS = {32A25 (33D70)},
	MRNUMBER = {3506300},
	MRREVIEWER = {Atsushi Yamamori},
	DOI = {10.1007/s11785-015-0505-4},
	URL = {https://doi.org/10.1007/s11785-015-0505-4},
}

@article {PJD13,
	AUTHOR = {Park, Jong-Do},
	TITLE = {Explicit formulas of the {B}ergman kernel for 3-dimensional
	complex ellipsoids},
	JOURNAL = {J. Math. Anal. Appl.},
	FJOURNAL = {Journal of Mathematical Analysis and Applications},
	VOLUME = {400},
	YEAR = {2013},
	NUMBER = {2},
	PAGES = {664--674},
	ISSN = {0022-247X},
	MRCLASS = {32A25 (32T27)},
	MRNUMBER = {3004995},
	MRREVIEWER = {Chunhui Qiu},
	DOI = {10.1016/j.jmaa.2012.11.017},
	URL = {https://doi.org/10.1016/j.jmaa.2012.11.017},
}

@article {BT15,
	AUTHOR = {Beberok, Tomasz},
	TITLE = {An explicit computation of the {B}ergman kernel function},
	JOURNAL = {Complex Var. Elliptic Equ.},
	FJOURNAL = {Complex Variables and Elliptic Equations. An International
	Journal},
	VOLUME = {60},
	YEAR = {2015},
	NUMBER = {8},
	PAGES = {1058--1067},
	ISSN = {1747-6933},
	MRCLASS = {32A25 (30C40 32A05)},
	MRNUMBER = {3350483},
	MRREVIEWER = {Atsushi Yamamori},
	DOI = {10.1080/17476933.2014.996214},
	URL = {https://doi.org/10.1080/17476933.2014.996214},
}

@misc{GCYY20,
	title={Comparison of invariant metrics on the symmetrized bidisc},
	author={Gunhee Cho and Yuan Yuan},
	year={arXiv:2004.04637 [math.DG], 2020},
	eprint={2004.04637},
	archivePrefix={arXiv},
	primaryClass={math.DG}
}

@article {CY80,
	AUTHOR = {Cheng, Shiu Yuen and Yau, Shing Tung},
	TITLE = {On the existence of a complete {K}\"{a}hler metric on noncompact
	complex manifolds and the regularity of {F}efferman's
	equation},
	JOURNAL = {Comm. Pure Appl. Math.},
	FJOURNAL = {Communications on Pure and Applied Mathematics},
	VOLUME = {33},
	YEAR = {1980},
	NUMBER = {4},
	PAGES = {507--544},
	ISSN = {0010-3640},
	MRCLASS = {53C55 (32F15 53C25 58G20)},
	MRNUMBER = {575736},
	MRREVIEWER = {Daniel M. Burns, Jr.},
	DOI = {10.1002/cpa.3160330404},
	URL = {https://doi.org/10.1002/cpa.3160330404},
}

@incollection {DKFJEHG84,
	AUTHOR = {Diederich, K. and Forn\ae ss, J. E. and Herbort, G.},
	TITLE = {Boundary behavior of the {B}ergman metric},
	BOOKTITLE = {Complex analysis of several variables ({M}adison, {W}is.,
	1982)},
	SERIES = {Proc. Sympos. Pure Math.},
	VOLUME = {41},
	PAGES = {59--67},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {1984},
	MRCLASS = {32H15 (32E35 32F15)},
	MRNUMBER = {740872},
	MRREVIEWER = {I. P. Ramadanov},
	DOI = {10.1090/pspum/041/740872},
	URL = {https://doi.org/10.1090/pspum/041/740872},
}
@article {DKFJE80,
	AUTHOR = {Diederich, Klas and Forn\ae ss, John Erik},
	TITLE = {Comparison of the {B}ergman and the {K}obayashi metric},
	JOURNAL = {Math. Ann.},
	FJOURNAL = {Mathematische Annalen},
	VOLUME = {254},
	YEAR = {1980},
	NUMBER = {3},
	PAGES = {257--262},
	ISSN = {0025-5831},
	MRCLASS = {32H15 (32F15)},
	MRNUMBER = {597082},
	MRREVIEWER = {B. Wong},
	DOI = {10.1007/BF01457999},
	URL = {https://doi.org/10.1007/BF01457999},
}


@article {AJLZYNJ18,
	AUTHOR = {Agler, Jim and Lykova, Zinaida A. and Young, N. J.},
	TITLE = {Algebraic and geometric aspects of rational {$\Gamma$}-inner
	functions},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {328},
	YEAR = {2018},
	PAGES = {133--159},
	ISSN = {0001-8708},
	MRCLASS = {32F45 (30E05 30J05 93B36 93B50)},
	MRNUMBER = {3771126},
	MRREVIEWER = {Steven George Krantz},
	DOI = {10.1016/j.aim.2017.12.018},
	URL = {https://doi.org/10.1016/j.aim.2017.12.018},
}

@article {WY18,
	AUTHOR = {Wu, Damin and Yau, Shing-Tung},
	TITLE = {Complete {K}\"{a}hler-{E}instein metrics under certain holomorphic
	covering and examples},
	JOURNAL = {Ann. Inst. Fourier (Grenoble)},
	FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
	VOLUME = {68},
	YEAR = {2018},
	NUMBER = {7},
	PAGES = {2901--2921},
	ISSN = {0373-0956},
	MRCLASS = {32Q15 (32H02 32Q20 32Q45 53C55)},
	MRNUMBER = {3959099},
	MRREVIEWER = {Azniv Kasparian},
	URL = {http://aif.cedram.org/item?id=AIF_2018__68_7_2901_0},
}


@article {WY20,
	AUTHOR = {Wu, Damin and Yau, Shing-Tung},
	TITLE = {Some negatively curved complex geometry},
	JOURNAL = {Proceedings of the 8th ICCM},
	FJOURNAL = {Proceedings of the 8th ICCM},
	VOLUME = {},
	YEAR = {2019},
	NUMBER = {},
	PAGES = {},
	ISSN = {},
	MRCLASS = {},
	MRNUMBER = {},
	DOI = {},
	URL = {},
}


@article {CDW89,
	AUTHOR = {Catlin, David W.},
	TITLE = {Estimates of invariant metrics on pseudoconvex domains of
	dimension two},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {200},
	YEAR = {1989},
	NUMBER = {3},
	PAGES = {429--466},
	ISSN = {0025-5874},
	MRCLASS = {32H15},
	MRNUMBER = {978601},
	MRREVIEWER = {K. T. Hahn},
	DOI = {10.1007/BF01215657},
	URL = {https://doi.org/10.1007/BF01215657},
}


@article{DY17,
	AUTHOR = {Damin Wu and Yau, Shing-Tung},
	TITLE = {Invariant metrics on negatively pinched complete Kähler manifolds},
	JOURNAL = {J. Amer. Math. Soc.},
	FJOURNAL = {Journal of the American Mathematical Society},
	VOLUME = {},
	YEAR = {2020},
	NUMBER = {33},
	PAGES = {103-133},
	ISSN = {1088-6834},
	MRCLASS = {Primary 32Q05, 32Q15, 32Q20, 32Q45; Secondary 32A25},
	MRNUMBER = {},
	MRREVIEWER = {},
	DOI = {10.1090/jams/933},
	URL = {https://doi.org/10.1090/jams/933},	
}

@article {JPDA94,
	AUTHOR = {D'Angelo, John P.},
	TITLE = {An explicit computation of the {B}ergman kernel function},
	JOURNAL = {J. Geom. Anal.},
	FJOURNAL = {The Journal of Geometric Analysis},
	VOLUME = {4},
	YEAR = {1994},
	NUMBER = {1},
	PAGES = {23--34},
	ISSN = {1050-6926},
	MRCLASS = {32H10},
	MRNUMBER = {1274136},
	MRREVIEWER = {Gregor Herbort},
	DOI = {10.1007/BF02921591},
	URL = {https://doi.org/10.1007/BF02921591},
}




@book {JP13,
	AUTHOR = {Jarnicki, Marek and Pflug, Peter},
	TITLE = {Invariant distances and metrics in complex analysis},
	SERIES = {De Gruyter Expositions in Mathematics},
	VOLUME = {9},
	EDITION = {extended},
	PUBLISHER = {Walter de Gruyter GmbH \& Co. KG, Berlin},
	YEAR = {2013},
	PAGES = {xviii+861},
	ISBN = {978-3-11-025043-5; 978-3-11-025386-3},
	MRCLASS = {32-02 (32F45)},
	MRNUMBER = {3114789},
	MRREVIEWER = {Viorel V\^{a}j\^{a}itu},
	DOI = {10.1515/9783110253863},
	URL = {https://doi.org/10.1515/9783110253863},
}




@incollection {NMY83,
	AUTHOR = {Mok, Ngaiming and Yau, Shing-Tung},
	TITLE = {Completeness of the {K}\"{a}hler-{E}instein metric on bounded
	domains and the characterization of domains of holomorphy by
	curvature conditions},
	BOOKTITLE = {The mathematical heritage of {H}enri {P}oincar\'{e}, {P}art 1
	({B}loomington, {I}nd., 1980)},
	SERIES = {Proc. Sympos. Pure Math.},
	VOLUME = {39},
	PAGES = {41--59},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {1983},
	MRCLASS = {53C55 (32F15 53C25)},
	MRNUMBER = {720056},
	MRREVIEWER = {Hung-Hsi Wu},
}



@incollection {HW93,
	AUTHOR = {Wu, H.},
	TITLE = {Old and new invariant metrics on complex manifolds},
	BOOKTITLE = {Several complex variables ({S}tockholm, 1987/1988)},
	SERIES = {Math. Notes},
	VOLUME = {38},
	PAGES = {640--682},
	PUBLISHER = {Princeton Univ. Press, Princeton, NJ},
	YEAR = {1993},
	MRCLASS = {32H15 (32-02 32H20 32L07)},
	MRNUMBER = {1207887},
	MRREVIEWER = {Antonella Nannicini},
}

@article {SKY09,
	AUTHOR = {Yeung, Sai-Kee},
	TITLE = {Geometry of domains with the uniform squeezing property},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {221},
	YEAR = {2009},
	NUMBER = {2},
	PAGES = {547--569},
	ISSN = {0001-8708},
	MRCLASS = {32Q15 (32F45 32G15)},
	MRNUMBER = {2508930},
	MRREVIEWER = {Makoto Masumoto},
	DOI = {10.1016/j.aim.2009.01.002},
	URL = {https://doi.org/10.1016/j.aim.2009.01.002},
}



@misc{GC18,
	title={Comparison of the Carathéodory-distance, the K\"ahler-Einstein distance and the Kobayashi-distance on complete Reinhardt domains},
	author={Gunhee Cho},
	year={arXiv:1806.06311 [math.DG], 2018},
	eprint={1806.06311},
	archivePrefix={arXiv},
	primaryClass={math.DG}
}



@article {GC19,
	AUTHOR = {Cho, Gunhee},
	TITLE = {Invariant Metrics on the Complex Ellipsoid},
	JOURNAL = {J Geom Anal.},
	FJOURNAL = {Journal of Geometric analysis},
	VOLUME = {},
	YEAR = {2019},
	NUMBER = {},
	PAGES = {},
	ISSN = {},
	MRCLASS = {},
	MRNUMBER = {},
	DOI = {10.1007/s12220-019-00333-w},
	URL = {https://doi.org/10.1007/s12220-019-00333-w},
}



@article {KMPF78,
	AUTHOR = {Klembeck, Paul F.},
	TITLE = {K\"{a}hler metrics of negative curvature, the {B}ergmann metric
	near the boundary, and the {K}obayashi metric on smooth
	bounded strictly pseudoconvex sets},
	JOURNAL = {Indiana Univ. Math. J.},
	FJOURNAL = {Indiana University Mathematics Journal},
	VOLUME = {27},
	YEAR = {1978},
	NUMBER = {2},
	PAGES = {275--282},
	ISSN = {0022-2518},
	MRCLASS = {32F15 (32H15 53C55)},
	MRNUMBER = {463506},
	MRREVIEWER = {Hung-Hsi Wu},
	DOI = {10.1512/iumj.1978.27.27020},
	URL = {https://doi.org/10.1512/iumj.1978.27.27020},
}

@book {GREKKTKSG11,
	AUTHOR = {Greene, Robert E. and Kim, Kang-Tae and Krantz, Steven G.},
	TITLE = {The geometry of complex domains},
	SERIES = {Progress in Mathematics},
	VOLUME = {291},
	PUBLISHER = {Birkh\"{a}user Boston, Ltd., Boston, MA},
	YEAR = {2011},
	PAGES = {xiv+303},
	ISBN = {978-0-8176-4139-9},
	MRCLASS = {32-02 (32A36 32M25 32M99 32Q45 32T15)},
	MRNUMBER = {2799296},
	MRREVIEWER = {Marek Jarnicki},
	DOI = {10.1007/978-0-8176-4622-6},
	URL = {https://doi.org/10.1007/978-0-8176-4622-6},
}
